The Fermi Paradox and the Aurora Effect: Exo-civilization Settlement, Expansion and Steady States

We model the settlement of the galaxy by space-faring civilizations in order to address issues related to the Fermi Paradox. We explore the problem in a way that avoids assumptions about the intent and motivation of any exo-civilization seeking to settle other planetary systems. We first consider the speed of an advancing settlement via probes of finite velocity and range to determine if the galaxy can become inhabited with space-faring civilizations on timescales shorter than its age. We also include the effect of stellar motions on the long term behavior of the settlement front which adds a diffusive component to its advance. The results of these models demonstrate that the Milky Way can be readily 'filled-in' with settled stellar systems under conservative assumptions about interstellar spacecraft velocities and launch rates. We then consider the question of the galactic steady-state achieved in terms of the fraction of settled planets. We do this by considering the effect of finite settlement civilization lifetimes on the steady states. We find a range of parameters for which the galaxy supports a population of interstellar space-faring civilizations even though some settleable systems are uninhabited. Both results point to ways in which Earth might remain unvisited in the midst of an inhabited galaxy. Finally we consider how our results can be combined with the finite horizon for evidence of previous settlements in Earth's geologic record. Our steady-state model can constrain the probabilities for an Earth visit by a settling civilization before a given time horizon. These results break the link between Hart's famous "Fact A" (no interstellar visitors on Earth now) and the conclusion that humans must, therefore, be the only technological civilization in the galaxy.

==> Galactic Settlement/bibliography.tex <==
%\bibliography{galactic_settlement.bib}
\begin{thebibliography}{}
\bibitem[Ashworth(2012)]{Ashworth2012} Ashworth, S.\ 2012, Journal of the British Interplanetary Society, 65, 140 

\bibitem[Ashworth(2014)]{Ashworth2014} Ashworth, S.\ 2014, Journal of the British Interplanetary Society, 67, 224 

\bibitem[Ball(1973)]{Ball1973} Ball, J.~A.\ 1973, \icarus, 19, 347 

\bibitem[Bj{\o}rk(2007)]{Bjork2007} Bj{\o}rk, R.\ 2007, International Journal of Astrobiology, 6, 89.

\bibitem[Bracewell(1960)]{Bracewell1960} Bracewell, R.~N.\ 1960, \nat, 186, 670.

\bibitem[Brin(1983)]{Brin1983} Brin, G.~D.\ 1983.\ The Great Silence - the Controversy Concerning Extraterrestrial Intelligent Life.\ Quarterly Journal of the Royal Astronomical Society 24, 283-309. 

\bibitem[Chyba, \& Hand(2005)]{ChybaHand} Chyba, C.~F., \& Hand, K.~P.\ 2005, \araa, 43, 31.

\bibitem[Cirkovic(2018)]{Cirkovic2018} Cirkovic, M.~M.\ 2018.\ The Great Silence: Science and Philosophy of Fermi's Paradox.\ The Great Silence: Science and Philosophy of Fermi's Paradox, Oxford University Press, Oxford, UK, ISBN: 9780199646302, 432 pp.\ .

\bibitem[Cotta, \& Morales(2009)]{Cotta2009} Cotta, C., \& Morales, A.\ 2009, Journal of the British Interplanetary Society, 62, 82.

\bibitem[Davies(2012)]{Davies2012} Davies, P.~C.~W.\ 2012.\ Footprints of alien technology.\ Acta Astronautica 73, 250-257. 

\bibitem[Davies(2011)]{Davies2011} Davies, P. C. W. 2011, The Eerie Silence: Renewing Our Search for Alien Intelligence (Orlando, FL: Mariner Books)

\bibitem[Drake(1965)]{Drake1965} Drake, F.~D.\ 1965, In Current Aspects of Exobiology, 323.

\bibitem[Forgan(2009)]{Forgan2009} Forgan, D.~H.\ 2009, International Journal of Astrobiology, 8, 121.

\bibitem[Frank(2018)]{Frank2018} Frank, A \ 2018.\ Light of the Stars. Alien Worlds and The Fate of the Earth.\ (W.W. Norton, New York) 

\bibitem[Freitas(1980)]{Freitas1980} Freitas, R.~A.\ 1980, Journal of the British Interplanetary Society, 33, 251.

\bibitem[Freitas(1985)]{Freitas1985} Freitas, R.~A.\ 1985, \icarus, 62, 518.

\bibitem[Hair \& Hedman(2013)]{Hair2013} Hair, T.~W., \& Hedman, A.~D.\ 2013, International Journal of Astrobiology, 12, 45 

\bibitem[Henry et al.(2018)]{Henry2018} Henry, T.~J., Jao, W.-C., Winters, J.~G., et al.\ 2018, \aj, 155, 265 

\bibitem[Galera et al.(2018)]{Galera2018} Galera, E., Galanti, G., \& Kinouchi, O. 2018. Invasion percolation solves Fermi Paradox but challenges SETI projects. International Journal of Astrobiology, 1-7. doi:10.1017/S1473550418000101


\bibitem[Gray(2015)]{Gray2015} Gray, R.,2015, The Fermi Paradox Is Neither Fermi’s Nor aParadox,” Astrobiology 15, no. 3195– 99.

\bibitem[Gros(2005)]{Gros05} Gros, C.\ 2005, Journal of the British Interplanetary Society, 58, 108.

\bibitem[Hart(1975)]{Hart1975} Hart, M.~H.\ 1975.\ Explanation for the Absence of Extraterrestrials on Earth.\ Quarterly Journal of the Royal Astronomical Society 16, 128. 

\bibitem[Haqq-Misra, \& Baum(2009)]{Haqq-Misra2009} Haqq-Misra, J.~D., \& Baum, S.~D.\ 2009, Journal of the British Interplanetary Society, 62, 47.

\bibitem[Haqq-Misra and Kopparapu(2012)]{Haqq-Misra2012} Haqq-Misra, J., Kopparapu, R.~K.\ 2012.\ On the likelihood of non-terrestrial artifacts in the Solar System.\ Acta Astronautica 72, 15-20. 

\bibitem[Jones(1976)]{Jones1976} Jones, E.~M.\ 1976, \icarus, 28, 421

\bibitem[Jones(1978)]{Jones1978} Jones, E.~M.\ 1978, Journal of the British Interplanetary Society, 31, 103 

\bibitem[Jones(1981)]{Jones1981} Jones, E.~M.\ 1981.\ Discrete calculations of interstellar migration and settlement.\ Icarus 46, 328-336.

\bibitem[Jones (1985)]{Jones1985}Eric M. Jones, 1985, Where Is Everybody?: An Account of Fermi’s Question (Los Alamos, NM: Los Alamos National Laboratory, 1985), http://www.fas.org/sgp/othergov/doe/lanl/la- 10311- ms.pdf.

\bibitem[Kinouchi(2001)]{Kinouchi2001} Kinouchi, O.\ 2001, arXiv e-prints , cond–mat/0112137.

\bibitem[Krugman(2010)]{Krugman2010} Krugman, P.\ 2010.\ The Theory of Interstellar Trade.\ Economic Inquiry 48, 1119-1123.

\bibitem[Kuiper, \& Morris(1977)]{Kuiper1977} Kuiper, T.~B.~H., \& Morris, M.\ 1977, Science, 196, 616

\bibitem[Landis(1998)]{Landis1998} Landis, G.~A.\ 1998, Journal of the British Interplanetary Society, 51, 163 

\bibitem[Lin, \& Loeb(2015)]{Lin2015} Lin, H.~W., \& Loeb, A.\ 2015, \apj, 810, L3.

\bibitem[Newman \& Sagan(1981)]{Newman1981} Newman, W.~I., \& Sagan, C.\ 1981, \icarus, 46, 293 

\bibitem[Robinson(2015)]{Robinson2015} Robinson, K.~S., Aurora, \ 2015, Orbit

\bibitem[Sagan \& Newman(1983)]{Sagan1983} Sagan, C., \& Newman, W.~I.\ 1983, \qjras, 24, 113 

\bibitem[Schmidt \& Frank(2018)]{SchmidtFrank2018}Schmidt, G., \& Frank, A. (2018). The Silurian hypothesis: Would it be possible to detect an industrial civilization in the geological record? International Journal of Astrobiology, 1-9

\bibitem[Siemion et al.(2013)]{Siemion2013} Siemion, A.~P.~V., and 10 colleagues 2013.\ A 1.1-1.9 GHz SETI Survey of the Kepler Field. I. A Search for Narrow-band Emission from Select Targets.\ The Astrophysical Journal 767, 94. 

\bibitem[Stull(1979)]{Stull1979} Stull, M.~A.\ 1979, Journal of the British Interplanetary Society, 32, 221

\bibitem[Tarter(2001)]{Tarter2001} Tarter, J.\ 2001.\ The Search for Extraterrestrial Intelligence (SETI).\ Annual Review of Astronomy and Astrophysics 39, 511-548. 

\bibitem[Tarter(2007)]{Tarter07} Tarter, J.~C.\ 2007, Highlights of Astronomy, 14, 14 

\bibitem[Tarter et al.(2010)]{Tarter2010} Tarter, J.~C., and 13 colleagues 2010.\ SETI turns 50: five decades of progress in the search for extraterrestrial intelligence.\ Instruments, Methods, and Missions for Astrobiology XIII 7819, 781902. 

\bibitem[Tipler(1980)]{Tipler1980} Tipler, F.~J.\ 1980, \qjras, 21, 267 

\bibitem[von Hoerner(1975)]{vonHoerner1975} von Hoerner, S.\ 1975, Journal of the British Interplanetary Society, 28, 691.

\bibitem[Vukoti{\'c}, \& {\'C}irkovi{\'c}(2012)]{Vukotic2012} Vukoti{\'c}, B., \& {\'C}irkovi{\'c}, M.~M.\ 2012. Astrobiological Complexity with Probabilistic Cellular Automata Origins of Life and Evolution of the Biosphere, 42, 347.

\bibitem[Walters et al.(1980)]{Walters1980} Walters, C., Hoover, R.~A., \& Kotra, R.~K.\ 1980, \icarus, 41, 193 

\bibitem[Webb(2002)]{Webb2002} Webb, S.\ 2002.\ If the universe is teeming with aliens...where is everybody?.\ If the universe is teeming with aliens...where is everybody?: fifty solutions to the Fermi paradox and the problem of extraterrestrial life/ Stephen Webb.~New York: Praxis Book/Copernicus Books, 2002.\ . 

\bibitem[Wiley(2011)]{Wiley2011} Wiley, K.~B.\ 2011.\ The Fermi Paradox, Self-Replicating Probes, and the Interstellar Transportation Bandwidth arXiv:1111.6131.

\bibitem[Wright et al.(2014)]{Wright2014} Wright, J.~T., Mullan, B., Sigurdsson, S., Povich, M.~S.\ 2014.\ The {\^G} Infrared Search for Extraterrestrial Civilizations with Large Energy Supplies. I. Background and Justification.\ The Astrophysical Journal 792, 26. 

\bibitem[Wright \& Oman-Reagan(2018)]{WrightOmanReagan2018} Wright, J.~T., \& Oman-Reagan, M.~P.\ 2018, International Journal of Astrobiology, 17, 177 

\bibitem[Wright(2018)]{Wright2018b} Wright, J.~T.\ 2018.\ Prior indigenous technological species.\ International Journal of Astrobiology 17, 96-100.

\bibitem[Wright et al.(2018)]{Wright2018a} Wright, J.~T., Kanodia, S., Lubar, E.\ 2018.\ How Much SETI Has Been Done? Finding Needles in the n-dimensional Cosmic Haystack.\ The Astronomical Journal 156, 260.

\bibitem[Zackrisson et al.(2015)]{Zackrisson2015} Zackrisson, E., Calissendorff, P., Asadi, S., \& Nyholm, A.\ 2015, \apj, 810, 23 

\end{thebibliography}
